Carbon Responder: Coordinating Demand Response for the Datacenter Fleet

The increasing integration of renewable energy sources results in fluctuations in carbon intensity throughout the day. To mitigate their carbon footprint, datacenters can implement demand response (DR) by adjusting their load based on grid signals. However, this presents challenges for private datacenters with diverse workloads and services. One of the key challenges is efficiently and fairly allocating power curtailment across different workloads. In response to these challenges, we propose the Carbon Responder framework. The Carbon Responder framework aims to reduce the carbon footprint of heterogeneous workloads in datacenters by modulating their power usage. Unlike previous studies, Carbon Responder considers both online and batch workloads with different service level objectives and develops accurate performance models to achieve performance-aware power allocation. The framework supports three alternative policies: Efficient DR, Fair and Centralized DR, and Fair and Decentralized DR. We evaluate Carbon Responder polices using production workload traces from a private hyperscale datacenter. Our experimental results demonstrate that the efficient Carbon Responder policy reduces the carbon footprint by around 2x as much compared to baseline approaches adapted from existing methods. The fair Carbon Responder policies distribute the performance penalties and carbon reduction responsibility fairly among workloads.

==> 05_results_bak.tex <==
\section{Experimental Evaluation}
\label{sec:experiment}

We evaluate DR policies, quantifying their ability to reduce carbon and examining the fairness of performance losses. First, we show DR dynamics by illustrating {\ourmodel}'s load adjustments during a representative day and detailing how rescheduling power usage reduces carbon and impacts performance (\S~\ref{sec:dynamics}). Then, we compare DR policies and show {\ourmodel} is more efficient than baselines, achieving greater carbon reductions with smaller performance penalties (\S~\ref{sec:efficiency}). Finally, we compare DR policies and show {\ourmodel} is more fair than baselines based on the dispersion of carbon reductions and performance penalties across workloads (\S~\ref{sec:perworkload}-\ref{sec:fairness}).

\subsection{Experimental Methods}

%With this data, \ourmodel learns performance penalty models, calculates load adjustment $\mathbf{D}$ for each policy, and reports resulting carbon reduction and performance impact.

First, \ourmodel models performance penalties resulting from power adjustments for each workload using equations \ref{eq:realcost} and \ref{eq:batchcost}. We use traces and data from four production workloads detailed in \S\ref{sec:data}. 

Second, we implement DR policies with optimization to determine load adjustment $\mathbf{D}$. We solve optimization problems with Scipy's Sequential Least Squares Programming. Optimization determines power adjustments for a two-day interval, allowing us to determine whether a policy delays batch jobs beyond 24 hours. Optimization is offline and day-ahead, which aligns with methods in prior work \cite{radovanovic_carbon-aware_2021}. We limit curtailments to at most half the workload's original power capacity entitlement, which accounts for the fact that idle power typically constitutes half of a server's total power usage and {\ourmodel} does not presently power down servers. 

Finally, we calculate carbon reductions for the two-day interval as the inner product of vectors for marginal carbon intensity and power reductions (\S\ref{sec:policies}). We process CAISO data to quantify marginal and average carbon intensity \cite{watttime_mer}. The datacenter's baseline operational carbon is at the scale of thousands of metric tons of $CO_2$ for the two-day interval. We assess policies against baselines, dividing carbon reduction by baseline carbon and dividing each workload's {\pce} implied by performance losses by its original \pce. 

%, based on the inner product of average carbon intensity and physical power usage
%We compare percentage changes in performance and carbon relative to the baseline values. 

\subsection{Carbon and Power Dynamics}
\label{sec:dynamics}
\begin{figure}
	\centering 
 \includegraphics[width=\columnwidth]{figures/power_usage_dr_.pdf} % first figure itself
	\vspace*{-.25in}
 \caption{Optimal power allocation of \ourmodel}
	\label{fig:ourmodel}
\end{figure}

Figure~\ref{fig:ourmodel} illustrates hourly marginal carbon intensity and power usage before and after \ourmodel. Lines present data for four workloads. Red and green areas between lines indicate negative and positive power adjustments, respectively. Adjustment $\mathbf{D}$ is calculated using CR1 and Optimization~\ref{eq:wo}. Collectively, the four workloads reduce operational carbon by 4.6\% and suffer a performance loss equivalent to a 4\% reduction in their power capacity.  

Real-time workloads reduce power usage (\textit{i.e.}, red adjustments) and degrade performance. \ig can tolerate reduced power and consistently curtails usage when carbon intensity is high, reducing carbon by 2.6\% and degrading performance by an equivalent of 2.9\% in power capacity. In contrast, \web suffers higher performance losses from DR and curtails usage less often, reducing carbon by only 0.4\% and degrading performance by an equivalent of 0.7\% in power capacity.

Batch workloads defer it (\textit{i.e.}, red and green adjustments), shifting power usage to hours of low carbon intensity. AI training and data pipeline workloads defer jobs from the 6pm--8am window to the 8am--6pm window, reducing carbon by $1.2\%$ and $0.3\%$ while degrading performance by only 0.2\% and 0.3\%. 

%Specifically, \ig reduces 2.6\% of total carbon footprint with a performance penalty equivalent to $2.9\%$ loss of datacenter \pce, whereas \web reduces only 0.4\% carbon footprint with a performance penalty of $0.7\%$. 

Figure~\ref{fig:ourmodel} visualizes outcomes from policy CR1 with $\lambda=6.9$. Other policies and settings could further reduce carbon or preserve performance. The next section sweeps hyperparameters for all policies to present carbon and performance trade-offs. 

%By sweeping this hyperparameter a trade-off curve can be obtained, shown as a purple line in Figure~\ref{fig:tradeoff}. The scenario represented by Figure~\ref{fig:ourmodel} is marked as a star in Figure~\ref{fig:tradeoff}.

\subsection{Demand Response Efficiency}
\label{sec:efficiency}
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/tradeoffCurves.pdf}	
   	\vspace*{-.25in}
\caption{Performance and carbon trade-off of Carbon Responder (CR) and the baseline approaches (B\#).}
	\label{fig:tradeoff}
\end{figure}

We evaluate the efficiency of carbon-informed DR based on its ability to reduce datacenter carbon while while mitigating performance degradation. By adjusting policies' hyperparameters (e.g., $\lambda$, cap\%, and $F$), we can obtain different DR outcomes and trade-offs between carbon and performance. 

Figure~\ref{fig:tradeoff} illustrates the Pareto frontiers of the baseline and \ourmodel policies. The x-axis represents carbon reductions, while the y-axis represents the total performance penalties incurred, both in percentage. Each policy is represented by an upward-sloping curve, indicating that as it reduce carbon more aggressively, performance degradation also increases. The policies located on the lower right of the figure achieve greater carbon reduction for the same level of performance loss, making them more efficient compared to those on the upper left.
For instance, when the performance loss ranges from 1\% to 5\%, CR1 achieves twice the carbon footprint reduction compared to the baseline schemes (B1-4).

Among the seven policies, CR1 exhibits the highest efficiency, followed by CR2 and B4 (the red line near the origin). This can be attributed to the fact that the weighted sum in optimization~\ref{eq:wo} is equivalent to minimizing carbon footprint under different performance penalty constraints, establishing a theoretical upper bound on efficiency. CR2 effectively minimizes the operational carbon footprint and performs well initially. However, as CR2 aggressively reduces carbon, the fairness constraint starts to limit its efficiency. Despite being less efficient than CR1, CR2 still outperforms B1 that caps power equally for every workload. While CR3 emphasizes fairness, it falls short in terms of efficiency, and its curve ramps up quickly. There is a trade-off between the efficiency of carbon reduction in DR and fairness. CR1 is efficient (global optimal) but unfair, CR2 is fairer in terms of performance penalties incurred, and CR3 utilizes rewards as decentralized incentives for carbon reduction but sacrifices efficiency.

B1, B2, and B3 are less efficient policies. Figure~\ref{fig:tradeoff} illustrates B1 without the batch preservation constraint; otherwise, B1 would have terminated at the yellow star. B3 initially outperforms B1 by curbing only RTS1, which is more resilient to power curtailment. However, B1 gradually surpasses B3 as the fixed human input priorities and SLOs of B2 start to limit its efficiency. Despite being performant, B2 incurs greater performance loss than B1 and B3 due to its additional objective of peak shaving and the extra constraint of batch preservation. On the other hand, B4 is highly efficient but not effective at all. It only curtails batch workloads in accordance with their SLOs, resulting in negligible performance impact and carbon reduction. This is because the batch workload without SLOs in our datacenter constitutes a small proportion.

\subsection{Service-level Analysis of DR Policies}
\label{sec:perworkload}
\begin{figure}%[h]
	\centering
	\includegraphics[width=\columnwidth]{figures/bwmulti_barchart_Perf.pdf}	  	
    \vspace*{-.25in}
\caption{Performance penalty per workload when the carbon reduction is 0.5, 2, and 8\%.}
\label{fig:bar1}
\end{figure}

\begin{figure}%[h]
	\centering
	\includegraphics[width=\columnwidth]{figures/bwmulti_barchart_Carb.pdf}	
   	\vspace*{-.25in}
\caption{Carbon reduction breakdown per workload when total performance penalty is 0.5, 2, and 8\%.}
\label{fig:bar2}
\end{figure}

To assess the distribution of DR responsibilities across workloads, Figures~\ref{fig:bar1} and \ref{fig:bar2} provide breakdowns of performance penalties and carbon reductions per workload for each policy. In Figure~\ref{fig:bar1}, the performance penalties per workload are shown for each policy, considering datacenter carbon reductions of 0.5\%, 2\%, and 8\%. Similarly, Figure~\ref{fig:bar2} shows the contribution of carbon reduction per workload for each policy, with datacenter performance penalties of 0.5\%, 2\%, and 8\%. The absence of bars for B3, B4, and CR3 in Figure~\ref{fig:bar1} and Figure~\ref{fig:bar2} indicate their incapability to achieve the specified carbon reduction or performance penalties.
% Similarly, 2\%, and 8\% of performance penalties are outside the range of B4 in Figure~\ref{fig:bar2}.

From Figure~\ref{fig:bar1}, 
% the x-axis represents the DR schemes, showcasing the fixed amount of carbon reduction achieved along with the corresponding performance penalties shown on the y-axis. The stacked bars in four different colors represent the four services in the datacenter.
CR1 achieves the theoretical minimum for the total performance penalty, as mentioned in Section~\ref{sec:efficiency}. Consequently, its bars represent the most efficient distribution of performance penalties.
In contrast, CR2 emphasizes fairness and imposes penalties based on the \pce of each workload. For instance, compared to CR1, CR2 allocates more penalties to \web than \ig because \web has a higher \pce. It is important to note that in CR2, AI training and data pipeline do not have performance penalties exactly proportional to their \pce due to constraints imposed by the batch preservation condition. While CR3 also prioritizes fairness, Figure~\ref{fig:bar1} does not reflect the fairness aspect of CR3. This is because CR3 emphasizes fairness in terms of the process of incentivizing DR, rather than focusing on the performance outcomes of DR.
% Although CR3 also focuses on fairness, it does not show its fairness aspect in Figure~\ref{fig:bar1} as it is not based on performance outcomes. Conversely, B1, B2, and B3 suffer significant performance losses.

Figure~\ref{fig:bar2} shows the breakdown of carbon reduction on the y-axis given three levels of fixed performance penalty. 
% In CR1, \ig and AI training contribute more to the total carbon reduction as they are more tolerant to degradation or delays. 
In CR2, the carbon reduction is more evenly distributed across workloads than CR1. Notably, in CR3, the carbon distribution follows the order of \pce for each workload. Despite the lower total carbon reduction, CR3 achieves the most fair allocation of the carbon reduction duty. 

The bar charts also provide insights into the performance of baseline policies in terms of efficiency and fairness. B1 applies proportional power capping and demonstrates fairness in both plots, but it lags in efficiency because power capping ignores the time-varying carbon intensities. B2 achieves similar efficiency but only curtails real-time workloads, leveraging their resilience toward power capping. On the other hand, B3 and B4 exclusively target either real-time or batch workloads for curtailment, leading to both unfair penalties and insufficient reduction of the carbon footprint.

% \begin{figure}%[h]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/barchart_Perf.pdf}	\caption{Performance penalty per workload when the carbon reduction is 2.5\% (except B4).}
% \label{fig:bar1}
% \end{figure}
% % \hl{remove captions above. multicolumns for each policy. fairness index on plots.}
% \begin{figure}%[h]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/barchart_Carb.pdf}	\caption{Carbon reduction breakdown per workload when total performance penalty is 5\% (except B4).}
% \label{fig:bar2}
% \end{figure}

\subsection{Fairness of DR Policies}
\label{sec:fairness}
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/entropy_boxplot.pdf}	
   	\vspace*{-.25in}
\caption{Normalized entropy of the carbon reduction and performance penalties across workloads of different policies.}
	\label{fig:entropy}
\end{figure}

To quantitatively assess whether each policy distributes power curtailments fairly across workloads, we show the Shannon entropies of the carbon breakdowns and performance penalties for each policy in Figure~\ref{fig:entropy}.
Shannon entropy is defined as $-\sum_{i=1}^n p_i \log p_i$ for a discrete distribution $p_i$. A higher entropy indicates a more fair result, with a maximum value of 2 when there are four workloads ($n=4$) and a uniform distribution. The entropy values in Figure~\ref{fig:entropy} are first scaled by the \pce of each workload: $p_i = {C_i}/{E_i} $ or $ {CF_i}/{E_i} $. If the performance penalties or carbon breakdowns of each workload are proportional to their \pce, the entropy reaches the maximum of 2. Thus, the left plot indicates how closely the carbon breakdown aligns with workloads' \pce, while the right plot demonstrates the proportionality of the performance penalty.

The box-and-whisker plots in depict the 1st quartile, median, and 3rd quartile of the entropies, with whiskers extending 1.5 times the inter-quartile range. From Figure~\ref{fig:entropy}, B1, CR2, and CR3 emerge as the most fair policies from both perspectives due to their equal treatment of workloads. B1 applies proportional caps to all workloads, resulting in fair DR, although it is not performance-optimized. CR2 and CR3 emphasize fairness in different aspects. CR2 incorporates fair outcome constraints, making it more fair in terms of performance outcomes. On the other hand, CR3 exhibits fairness in the carbon breakdown because it utilizes carbon reduction as the incentive to motivate workloads. B2 and CR1 demonstrate similar entropy values as they are both optimization-based and lack fairness considerations. In contrast, B3 and B4 rank as the least fair policies as they discriminate and curtail workloads based on their types.



==> 06_realizing_DR.tex <==
% \section{Incentivizing DR}
\section{Realizing Demand Response}
\hl{The whole section is new.}

\ourmodel provides different approaches to realize the load adjustment plans.
The optimization formulations and results also differ depending on how to enforce or incentivize the workloads to participate. 

% \hl{Todo: The fairness notion to motivate the three options. Rename the options to xxx fairness.}
% there are Directly Enforced DR, Fairly Enforced DR, and Payment Motivated DR.

\textbf{Efficient DR} directly enforces the centralized global optimal load adjustment.
To enforce the load adjustment, \ourmodel can levy tax only on those workloads not following the provided load adjustment $\vec d_i$ plans. In this way the workloads are forced to adjust \ppu to the degree of the punishment and the tax determines the performance degradation which workloads are willing to undergo. For example, when \ig is taxed 10.33 \np \pce if not participating, it would accept the load adjustment plans $\vec d_i$ with $c_i(\vec d_i) \leq 10.33$ \np as in Figure~\ref{fig:ourmodel}.
This approach achieves the optimally calculated performance penalties but is punishment-driven and is not fair to workloads. Optimization~\ref{eq:bar} and \ref{eq:wo} in Section~\ref{sec:experiment} are Efficient DR.


% When applying tax, workloads are allowed to utilize more than their \pce as long as the whole datacenter capacity is not exceeded:

\textbf{Fair Outcome DR} enforces an equal performance degradation on workloads.
Similar to Efficient DR, tax can be levied but with the same rate across workloads to degrade performance fairly. It sacrifices efficiency because it ignores the inter-workload optimization.
The result of equal tax rate (10\%) upon all workloads is shown in figure~\ref{fig:opt_equal_tax_10}. Different weights do not change the optimal load adjustment or carbon reduction in this case because there is no inter-workload comparison, each workload independently performs DR up till the performance cost equals to the fair punishment.  Optimization~\ref{eq:cn} and \ref{eq:bdr} in Section~\ref{sec:experiment} are Fair Outcome DR.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/opt_equal_tax_10.pdf} % first figure itself
	\caption{Load adjustments for 10\% performance degradation}
	\label{fig:opt_equal_tax_10}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/lambda_opts_weights5.pdf} % first figure itself
	\caption{\hl{Effectiveness of Different Approaches}}
	\label{fig:lambda3opt}
\end{figure}

\textbf{Fair Opportunity DR} is a decentralized, payment motivated DR as opposed to the first two. It confiscates equal share of \pce and then pays workloads to incentivize the carbon reduction.
Hence, each workload has equal opportunity to earn \pce back by participating in the DR. In addition to fair payment, it uses decentralized optimization. The first two options optimize at the fleet level and allocate the $d$ to directly minimizes carbon footprint and total performance loss while bypassing the individual workloads' interests. However, a participatory framework would have each workload optimizes for their own good with fair opportunities.

% However, when optimization is shifted to individual workloads, or when it becomes a bilevel programming \cite{talari_optimal_2019}, the carbon footprint is no longer an exogenous target, but a part of the workload's utility.

\textbf{Mathematical Formulation of Payment.} 
$\vec d_{i, s}$ is still the load adjustment vector of $i$ at day $s$, i.e., a delta of $\ppu_i$ before and after applying \ourmodel.
Let the $T_{i, s}$ and $P_{i, s}$ denote the tax paid and the compensation received by workload $i$ at day $s$, respectively. Let $\pce_{i}$ be the \pce of $i$ without applying \ourmodel, assuming it constant over time. $\pce_{i} - T_{i, s} + P_{i, s}$ is thus the realized \pce after adjusting for tax and compensation.
% \begin{equation}
% \label{eq:dcpce}
%     \max_s \sum_i ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \text{Datacenter Capacity}
% \end{equation}
This \pce constraints prevent workload from using more power than their entitlement (after adjusted by tax and compensation):
\begin{equation}
\label{eq:pce}
    \max ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \pce_i - T_{i, s} + P_{i, s}
\end{equation}
where if $T_{i, s} > P_{i, s}$ there will be a performance penalty from tax, as in Figure~\ref{fig:pceshaving}. Let the $\bar c_{i} (\pce_{i} - T_{i, s} + P_{i, s})$ denote this cost due to \pce shrinking/capping when DR is absent. 
The tax equality constraint makes sure the datacenter has fiscal balance. i.e., all compensations payed at day $s$ are covered by tax levied:
\begin{equation}
\label{eq:fiscal}
    \sum_i T_{i,s} \geq \sum_i P_{i,s}
\end{equation}

Assuming constraints~\ref{eq:pce} and~\ref{eq:fiscal}, a decentralized DR can be formulated as the bilevel programming problem:
\begin{equation}
	\begin{aligned}
		\label{eq:bilevel}
		& \min_{P_i(\vec d_i), T_i} \ CF(\vec D_{i}) \\
		& s.t. \ \vec d_i \in \arg \min C_i(\vec d_i) \\ & \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation}
where the outer (upper) level is the fleet trying to reduce carbon footprint with a correct payment function $P_i(\vec d_i)$, while the inner level is each individual workload minimizing the performance loss incurred due to tax $T_i$ with payment from DR.
For simplicity, let payment be the carbon reduction $P_i(\vec d_i) = CF(\vec d_i)$ and $T_i = 20\% \pce_i$. The workload level optimization gives us Figure~\ref{fig:innerlevel}. 
\begin{equation}
	\begin{aligned}
		\label{eq:innerlevel}
		& \min_{\vec d_i} \ C_i(\vec d_i)  \\ 
		& s.t. \ P_i(\vec d_i) = CF(\vec d_i) , \ T_i = 0.2\ \pce_i
		\\ &  \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation} 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/equilibrium3} % first figure itself
	\caption{Optimal Load Adjustment at Workload Level}
	\label{fig:innerlevel}
\end{figure}
In this case, all payment are chosen by each workload for their own good. 
% The net tax paid by each workload are [1.68 2.31 -1.11 0.36]. The fiscal balance is 3.23 \pce, performance cost is 14.75 with 1.6\% carbon reduction, as shown in Figure~\ref{fig:innerlevel}. When tax rate is 10\%, the net tax paid are [1.4138 1.9557 0.6607 3.3118] total 7.34 and the total cost is 1.89 with carbon reduce 0.56\%.
When the tax collected is not fully utilized, each workload is independently at its optimal DR/payment level, i.e., the marginal benefit of performing more DR is zero. However, after all tax is paid back as compensation, workloads could benefit from performing more DR but end up constrained by equation~\ref{eq:fiscal}.
% tax rate and the $C$. Also can find the optimal tax rate. 

\textbf{Effectiveness of DR Options.}
There is a trade-off between the efficiency of DR at carbon reduction and the enforcement difficulty. Figure~\ref{fig:lambda3opt} plots the Pareto frontiers of different options, where the x axis is the carbon reductions and the y axis is the total performance penalties incurred. The frontiers on the left reduce more carbon emission given the same performance loss: Efficient DR is efficient (global optimal) but unfair; Fair Outcome DR is more fair for the performance penalties incurred; Fair Opportunity DR uses rewards rather than punishment to incentivize the carbon reduction, but less efficient.



==> background_table.tex <==

\begin{table*}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{0.24 \linewidth} | p{0.18\linewidth} | p{0.1\linewidth}  p{0.1\linewidth}  p{0.1\linewidth}  p{0.1\linewidth} | p{0.15\linewidth} }

\hline
\multirow{2}{*}{DR Frameworks} &
  \multicolumn{1}{c|}{Objective} &
  \multicolumn{4}{c|}{Allocation} &
  \multicolumn{1}{c}{Enforcing Mechanism} \\ \cline{2-7} 
 &
  Objective functions to minimize   &
  \multicolumn{1}{p{0.1\linewidth}|}{DR on batch workloads} &
  \multicolumn{1}{p{0.1\linewidth}|}{DR on realtime workloads} &
  \multicolumn{1}{p{0.1\linewidth}|}{Across-workload apportioning} &
  Modeling the performance impact&
  Fairness policies\\ \hline
Google CA DR 
  \cite{radovanovic_carbon-aware_2021} &
  Carbon \& peak power  &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
   &
   \\ \hline
Dynamo 
  \cite{wu_dynamo_2016} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
   &
   \\ \hline
Throttling 
  \cite{govindan_benefits_2011} &
  Peak power &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
   \\ \hline
OLDI Power Mangement 
  \cite{meisner_power_2011} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
   \\ \hline
QoS Assurance DR 
  \cite{zhang_hpc_2022} &
   &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark} &
   \\ \hline
% UCB Technical Report 
%   \cite{krioukov_design_2012} &
%   Carbon or energy cost &
%   \multicolumn{1}{c|}{\checkmark} &
%   \multicolumn{1}{c|}{\checkmark} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{\checkmark} &
%    \\ \hline
\ourmodel &
  Carbon \& perf loss &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c}{\checkmark} \\ \hline
\end{tabular}%
}
\caption{Related Work and \ourmodel}
\label{tab:baselines}
\end{table*}

==> dynamics.tex <==
\section{Incentivizing DR}
In previous sections, \ourmodel calculates and enforces the optimal load adjustment $\vec d_i$ for each workload $i$. There are different approaches to realize the load adjustment plans.

\subsection{Tax Motivated DR}
To incentivize the load adjustment, \ourmodel can levy tax only on those workloads not following the provided load adjustment $\vec d_i$ plans. In this way the workloads are forced to adjust \ppu to the degree of the taxed \pce. i.e., the tax determines the performance degradation which workloads are willing to undergo. For example, when \ig is taxed 10 \np \pce if not participating, it would accept the load adjustment plans $\vec d_i$ with $c_i(\vec d_i) \leq 10$ \np.

This approach is the tax motivated DR. Tax can be equally levied with same tax rate across workloads, or it can be optimally calculated as in previous sections.

When applying tax, workloads are allowed to utilize more than their \pce as long as the whole datacenter capacity is not exceeded:
\begin{equation}
\label{eq:dcpce}
    \max_s \sum_i ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \text{Datacenter Capacity}
\end{equation}
The result of equal tax rate (10\%) upon all workloads is shown in figure~\ref{fig:opt_equal_tax_10}. Different weights do not change the optimal load adjustment or carbon reduction in this case because weights only show up on both sides of the cost neutral constraints $ c_i(\vec d_i) = c_i(\pce_i - T_i) , \ \forall i$. i.e., there is no inter-workload comparison or optimization, each workload independently performs DR up till the performance cost equals to its tax incurred cost. 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/opt_equal_tax_10.pdf} % first figure itself
	\caption{Load adjustments for 10\% tax}
	\label{fig:opt_equal_tax_10}
\end{figure}

\subsection{Payment Motivated DR}
Another approach is payment motivated approach. 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/lambda3opt} % first figure itself
	\caption{Effectiveness of Different Approaches}
	\label{fig:lambda3opt}
\end{figure}

% \subsection{Optimal DR at Workload Level}
Note that in previous cases, the optimizations above still happen at the fleet level, that allocates the $d$ to directly minimizes carbon footprint and total performance loss while bypassing the individual workloads' interests. A realistic framework would have each workload optimizes for their own good. 

However, when optimization is shifted to individual workloads, or when it becomes a bilevel programming \cite{talari_optimal_2019}, the carbon footprint is no longer an exogenous target, but a part of the workload's utility.

\paragraph{Mathematical Formulation.} 
Let the $T_{i, s}$ and $P_{i, s}$ denote the tax paid and the compensation received by workload $i$ at day $s$, respectively. Let $\pce_{i}$ be the \pce of $i$ without applying \ourmodel, assuming it constant over time. $\pce_{i} - T_{i, s} + P_{i, s}$ is thus the realized \pce after adjusting for tax and compensation.
This \pce constraints prevent workload from using more power than their entitlement (after adjusted by tax and compensation):
\begin{equation}
\label{eq:pce}
    \max ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \pce_i - T_{i, s} + P_{i, s}
\end{equation}
where if $T_{i, s} > P_{i, s}$ there will be a performance penalty from tax, as in Figure~\ref{fig:pceshaving}. Let the $\bar c_{i} (\pce_{i} - T_{i, s} + P_{i, s})$ denote this cost due to \pce shrinking/capping when DR is absent. 

$\vec d_{i, s}$ is still the load adjustment vector of $i$ at day $s$, i.e., a delta of $\ppu_i$ before and after applying \ourmodel.

The tax equality constraint makes sure the datacenter has fiscal balance. i.e., all compensations payed at day $s$ are covered by tax levied:
\begin{equation}
\label{eq:fiscal}
    \sum_i T_{i,s} \geq \sum_i P_{i,s}
\end{equation}

Assuming again constraints~\ref{eq:pce} and~\ref{eq:fiscal}, but now having the bilevel programming problem:

\begin{equation}
	\begin{aligned}
		\label{eq:bilevel}
		& \min_{P_i(\vec d_i), T_i} \ CF(\vec D_{i}) \\
		& s.t. \ \vec d_i \in \arg \min C_i(\vec d_i) \\ & \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation}
where the outer (upper) level is the fleet trying to reduce carbon footprint with a correct payment function $P_i(\vec d_i)$, while the inner level is each individual workload minimizing the performance loss incurred due to tax $T_i$ with payment from DR.

For simplicity, let $P_i(\vec d_i) = CF(\vec d_i)$ and $T_i = 20\% \pce_i$. The workload level optimization gives us: 
\begin{equation}
	\begin{aligned}
		\label{eq:innerlevel}
		& \min_{\vec d_i} \ C_i(\vec d_i)  \\ 
		& s.t. \ P_i(\vec d_i) = CF(\vec d_i) , \ T_i = 0.2\ \pce_i
		\\ &  \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation} 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/equilibrium3} % first figure itself
	\caption{Optimal Load Adjustment at Workload Level}
	\label{fig:innerlevel}
\end{figure}
In this case, all payment are chosen by each workload for their own good. The net tax paid by each workload are [1.68 2.31 -1.11 0.36]. The fiscal balance is 3.23 \pce, performance cost is 14.75 with 1.6\% carbon reduction, as shown in Figure~\ref{fig:innerlevel}. When tax rate is 10\%, the net tax paid are [1.4138 1.9557 0.6607 3.3118] total 7.34 and the total cost is 1.89 with carbon reduce 0.56\%.

When the tax collected is not fully utilized, each workload is independently at its optimal DR/payment level, i.e., the margin benefit of \pce compensation from performing DR is zero. However, after all tax paid back as compensation, workloads could benefit from performing more DR but end up constrained by equation~\ref{eq:fiscal}.
% tax rate and the $C$. Also can find the optimal tax rate. 


\begin{table*}[]
	\centering
	\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l}
	\hline
	Services                                                                 & Description                                                                                                                              & Category* & SLAs                                                                                       \\ \hline
	AI Research (FAIR)                                                              & 3rd party GPU clusters for AI researchers                                                                                                & Batch     & No SLA                                                                                     \\ \hline
	\begin{tabular}[c]{@{}l@{}}Elastic Compute\\ High Availability\end{tabular} & \begin{tabular}[c]{@{}l@{}}The required capacity is allocated in each 1 \\ day window and is met on average\end{tabular}                 & Elastic   & No SLA                                                                                     \\ \hline
	\begin{tabular}[c]{@{}l@{}}Elastic Compute \\ Opportunistic\end{tabular}    & \begin{tabular}[c]{@{}l@{}}These reservation has no fulfillment guarantees \\ and will be allocated whenever supply permits\end{tabular} & Elastic   & No SLA                                                                                     \\ \hline
	Data warehouse                                                                  & \begin{tabular}[c]{@{}l@{}}Storing and querying data. Writing, \\ scheduling, and deploying batch data pipelines.\end{tabular}           & Batch     & \begin{tabular}[c]{@{}l@{}}Five tiers of SLAs: \\ 1,2,4,8 and $\infty$ hours.\end{tabular} \\ \hline
	Ads                                                                      & Serving Ads via ML model inference                                                                                                       & Online    & realtime                                                                                   \\ \hline
	AI Infra (MAST)                                                                 & AI model training cluster for production                                                                                                 & Batch     & No SLA                                                                                     \\ \hline
	Web                                                                      & Serving real-time traffic for Web app clients                                                                                            & Online    & realtime                                                                                   \\ \hline
	Instagram Realtime                                                             & Real-time jobs of APP. Most of Instagram traffic is here.                                                                                      & Online    & realtime                                                                                   \\ \hline
	Instagram Async                                                                & Async Instagram jobs running on a special serverless tier                                                                                      & Elastic   & 4 hour                                                                                     \\ \hline
	Async Reserved                                                      & A group of delay-intolerant serverless jobs                                                                                              & Online    & 3 seconds                                                                                  \\ \hline
	Async Shared                                                        & A group of delay-tolerant serverless jobs                                                                                                & Elastic   & 24 hours                                                                                   \\ \hline
\end{tabular}%
	}
\caption{\meta Workload}
\label{tab:workload}
\end{table*}


\if 0
% \ifx\mycmd\undefined
\section{Endogenous Compensations}
In this section we introduce the constraint of \pce in DR, and analysis how the compensation in \ourmodel is collected and spent, and the dynamics thereafter.

\paragraph{Mechanism of tax and compensation of \pce.}
\ourmodel enforces that each workload can not use more power than their PCE (Equation~\ref{eq:pce}). \ourmodel levies tax upon \pce (in unit of \np) of all workloads, and then use the levied \pce to pay back the compensation of DR program promised in the last time window. In this case the performance cost could come from two sources, 1). the DR-incurred performance cost, which equals to the compensation, and 2). the tax-incurred performance cost, which is not compensated by \ourmodel. 

\paragraph{Mathematics Formulation.} Let the $T_{i, s}$ and $P_{i, s}$ denote the tax paid and the compensation received by workload $i$ at day $s$, respectively. Let $\pce_{i}$ be the \pce of $i$ without applying \ourmodel, assuming it constant over time. $\pce_{i} - T_{i, s} + P_{i, s}$ is thus the realized \pce after adjusting for tax and compensation.
This \pce constraints prevent workload from using more power than their entitlement (after adjusted by tax and compensation):
\begin{equation}
\label{eq:pce}
    \max ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \pce_i - T_{i, s} + P_{i, s}
\end{equation}
where if $T_{i, s} > P_{i, s}$ there will be a performance penalty from tax, as in Figure~\ref{fig:pceshaving}. Let the $\bar c_{i} (\pce_{i} - T_{i, s} + P_{i, s})$ denote this cost due to \pce shrinking/capping when DR is absent. 

$\vec d_{i, s}$ is still the load adjustment vector of $i$ at day $s$, i.e., a delta of $\ppu_i$ before and after applying \ourmodel. However, the compound performance cost $c_i(\vec d_i)$ can be decomposed as the sum of two terms, the DR-incurred performance cost and the tax-incurred performance cost: $c_i(\vec d_i) = \left[ c_{i} ( \vec d_{i} ) - \bar c_{i} (\pce_{i} - T_{i, s} + P_{i, s}) \right] + \bar c_{i} (\pce_{i} - T_{i, s} + P_{i, s})$. \ourmodel only compensates the first term. Thus, the compensation $P_{i, s+1}$ workload $i$ receives the next day is
\begin{equation}
\label{eq:compensation}
    P_{i, s+1} (T_{i, s}, P_{i, s}, \vec d_{i, s}) = c_{i, s} ( \vec d_{i, s} ) - \bar c_{i, s} (\pce_{i} - T_{i, s} + P_{i, s})
\end{equation}

The tax equality constraint makes sure the datacenter has fiscal balance. i.e., all compensations payed at day $s$ are covered by tax levied:
\begin{equation}
\label{eq:fiscal}
    \sum_i T_{i,s} \geq \sum_i P_{i,s}
\end{equation}

As for the tax, \ourmodel levies it proportionally to the PCE: $T_{i,s} \propto \pce_i$, but the tax rate is calculated within the optimization framework to make Equation~\ref{eq:fiscal} hold.

\subsection{Solving for Comparative Equilibrium}

Now to simplify the dynamic system, we let $P_{i, s+1} = P_{i, s}$ and solve for the fixed point. Following  Optimization~\ref{eq:bar}, but with more constraints~\ref{eq:compensation}, \ref{eq:fiscal}, and \ref{eq:pce}. The tax rate will be $3.9\%$ and the result is shown in Figure~\ref{fig:endogonous2}. The net tax paid by each workload: $ T_{i,s}  - P_{i,s} = $ [-1.8690 -1.9891 0.9214 2.9366], indicating that AI Infra and Storage have a \pce reduction after paying tax. Even though \ig and Web also pay tax, their \pce increase because of the compensation of DR.

The performance costs due to tax (not compensated) is $ \bar c_{i,s} = $ [6.6436 7.2139 0.1551 0.2910], roughly twice of that due to DR (compensated): [3.6696 4.2598 0.0667 0.1226]. They sum up to be the total performance cost shown in Figure~\ref{fig:endogonous2}.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/equilibrium2} % first figure itself
	\caption{Load adjustments for 5\% carbon reduction}
	\label{fig:endogonous2}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/equilibrium} % first figure itself
	\caption{Load adjustments when $\lambda = 1$ for Optimization~\ref{eq:wo}}
	\label{fig:endogonous}
\end{figure}

We can also do it with Optimization~\ref{eq:wo}.
When $\lambda = 1$, the result is shown in Figure~\ref{fig:endogonous}. The optimal tax is calculated as $T_i = 9.2\% \times \pce_i$, and the tax levied is $T_{i,s} = $ [4.2699 5.3850 2.3434 7.2547] for 4 workloads, the net tax is $ T_{i,s}  - P_{i,s} = $ [-3.0021 -4.0872 1.0283 6.0610]. The cost due to DR (also the compensation) of each workload: $P_{i,s} = $ [7.2720 9.4722 1.3151 1.1937].
In this special case in Figure~\ref{fig:endogonous}, there would have been a large performance degradation from levying the \pce, $\bar c_{i,s} = $ [43.9346 49.1760 7.9901 10.0397]. More than 6 times the actually compensation.

\subsection{Cost Neutral at Workload Level}
To make full use of the payment and to neutralize the cost of participation of DR for each workload, we combine Optimization~\ref{eq:cn} with constraints~\ref{eq:compensation}, \ref{eq:fiscal}, \ref{eq:pce}, and let the cost of each workload equals to the no DR scenario:  $ c_i(\vec d_i) = c_i(\pce_i - T_i+P_i) $. This and constraint~\ref{eq:compensation} implies that there will be no compensations. The performance costs due to tax: [0.7069 1.0239 0.1077 0.1969] is same as the realized performance loss from DR. In this way the incentives are matched. Tax rate is $3.6\%$ and under this tax rate the cost of DR is same as the cost of merely paying the tax.

Different weights do not change the optimal tax rate, load adjustment or carbon reduction in this case because weights only show up on both sides of the cost neutral constraints $ c_i(\vec d_i) = c_i(\pce_i - T_i+P_i) , \ \forall i$. i.e., there is no inter-workload comparison or optimization, each workload independently performs DR up till the performance cost equals to its tax incurred cost. The total performance cost is 2.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/equilibrium4} % first figure itself
	\caption{Load adjustments for Workload Cost Neutral}
	\label{fig:innerlevel}
\end{figure}

To make the cost of DR indifferent from that of tax, the constraint~\ref{eq:pce} can be loosen to allow workload to utilize more than their \pce as long as the whole datacenter capacity is not exceeded:
\begin{equation}
\label{eq:dcpce}
    \max_s \sum_i ( \vec{\ppu}_{i,s} - \vec d_{i,s} ) \leq \text{Datacenter Capacity}
\end{equation}

\subsection{Optimal DR at Workload Level}
Note that in both cases, the net tax paid is positive for both \ig and Web, but the compensation are not utilized to bring any benefits. That is because the optimizations above still happen at the fleet level, that allocates the $d$ to directly minimizes carbon footprint and total performance loss while bypassing the individual workloads' interests. A realistic framework would have each workload optimizes for their own good. 

However, when optimization is shifted to individual workloads, or when it becomes a bilevel programming \cite{talari_optimal_2019}, the carbon footprint is no longer an exogenous target, but a part of the workload's utility.

\paragraph{Mathematical Formulation.} Assuming again constraints~\ref{eq:pce} and~\ref{eq:fiscal}, but now having the bilevel programming problem:

\begin{equation}
	\begin{aligned}
		\label{eq:bilevel}
		& \min_{P_i(\vec d_i), T_i} \ CF(\vec D_{i}) \\
		& s.t. \ \vec d_i \in \arg \min C_i(\vec d_i) \\ & \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation}
where the outer (upper) level is the fleet trying to reduce carbon footprint with a correct payment function $P_i(\vec d_i)$, while the inner level is each individual workload minimizing the performance loss incurred due to tax $T_i$ with payment from DR.

For simplicity, let $P_i(\vec d_i) = CF(\vec d_i)$ and $T_i = 20\% \pce_i$. The workload level optimization gives us: 
\begin{equation}
	\begin{aligned}
		\label{eq:innerlevel}
		& \min_{\vec d_i} \ C_i(\vec d_i)  \\ 
		& s.t. \ P_i(\vec d_i) = CF(\vec d_i) , \ T_i = 0.2\ \pce_i
		\\ &  \text{and constraints~\ref{eq:pce} and~\ref{eq:fiscal}} 
	\end{aligned}
\end{equation} 

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{asplos23-templates-summer-2/figures/equilibrium3} % first figure itself
	\caption{Optimal Load Adjustment at Workload Level}
	\label{fig:innerlevel}
\end{figure}
In this case, all payment are chosen by each workload for their own good. The net tax paid by each workload are [1.68 2.31 -1.11 0.36]. The fiscal balance is 3.23 \pce, performance cost is 14.75 with 1.6\% carbon reduction. When tax rate is 10\%, the net tax paid are [1.4138 1.9557 0.6607 3.3118] total 7.34 and the total cost is 1.89 with carbon reduce 0.56\%.

Notice here the tax seems not to be fully utilized. Can explore the relationship between tax rate and the $C$. Also can find the optimal tax rate. 

\fi
